Indaleko: The Unified Personal Index

Personal information retrieval fails when systems ignore how human memory works. While existing platforms force keyword searches across isolated silos, humans naturally recall through episodic cues like when, where, and in what context information was encountered. This dissertation presents the Unified Personal Index (UPI), a memory-aligned architecture that bridges this fundamental gap. The Indaleko prototype demonstrates the UPI's feasibility on a 31-million file dataset spanning 160TB across eight storage platforms. By integrating temporal, spatial, and activity metadata into a unified graph database, Indaleko enables natural language queries like "photos near the conference venue last spring" that existing systems cannot process. The implementation achieves sub-second query responses through memory anchor indexing, eliminates cross-platform search fragmentation, and maintains perfect precision for well-specified memory patterns. Evaluation against commercial systems (Google Drive, OneDrive, Dropbox, Windows Search) reveals that all fail on memory-based queries, returning overwhelming result sets without contextual filtering. In contrast, Indaleko successfully processes multi-dimensional queries combining time, location, and activity patterns. The extensible architecture supports rapid integration of new data sources (10 minutes to 10 hours per provider) while preserving privacy through UUID-based semantic decoupling. The UPI's architectural synthesis bridges cognitive theory with distributed systems design, as demonstrated through the Indaleko prototype and rigorous evaluation. This work transforms personal information retrieval from keyword matching to memory-aligned finding, providing immediate benefits for existing data while establishing foundations for future context-aware systems.

==> latexmkrc <==
$pdflatex = 'xelatex -file-line-error %O %S';
$pdf_mode = 4;

add_cus_dep( 'acn', 'acr', 0, 'makeglossaries' );
add_cus_dep( 'glo', 'gls', 0, 'makeglossaries' );
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

$clean_ext .= " acr acn alg ddf glo gls glg bbl xdy xwm glsdefs run.xml";
sub makeglossaries {
  my ($base_name, $path) = fileparse( $_[0] );
  pushd $path;
  my $return = system "makeglossaries", $base_name;
  popd;
  return $return;
}

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR XELATEX
        system( "latexmk -cd -xelatex \"$_[0]\"" );
   }
}

@default_excluded_files = ('terms.tex');
@default_files=('diss');

